Sum-product phenomena: p-adic case

The sum-product phenomena over a finite extension K of $\mathbb{Q}_p$ is explored. The main feature of the results is the fact that the implied constants are independent of $p$.

==> SG_StructureOfGrades.tex <==
\subsection{Graded structure of sum-product subsets.}
In this section we study the structure of $\gr_i \gen{A}{C}$.  Let us start with (a variation of) \cite[Theorem~4]{BKT}. We include the proof for the convenience of the reader. 
\begin{lem}\label{l:BoundedGenerationFiniteField}
For any $0<\vare\ll 1$, positive integer $C\gg_{\vare} 1$, and a finite field $\f$ the following holds: 

Suppose $B\subseteq \f$, $|B|\ge |\f|^{\vare}$, and $0,1\in B$. Then $\gen{B}{C}$ is a subfield of $\f$. 
\end{lem}
\begin{proof}
By \cite[Lemma 4.1]{BKT}, there are $\alpha_1,\ldots,\alpha_k\in \f^{\times}$ such that $k\ll_{\vare} 1$ and 
\[
\alpha_1 B+\cdots+\alpha_k B=\f.
\]
{\bf Claim 1:} {\em Suppose $0,1\in X\subseteq \f$ and $\alpha_i\in \f^{\times}$ such that 
\be\label{ce:BoundedGenerationFiniteField}
\f=\alpha_1 X+\cdots+\alpha_k X.
\ee
Then either we have {\bf (reduction)}
$
\f=\sum_{i\neq i_0} \alpha_i \gen{X}{2},
$
for some $i_0$, or {\bf (injectivity)} for any $\xbf,\xbf'\in X^k$
$
\sum_i \alpha_i x_i=\sum_i \alpha_i x_i' \Rightarrow \xbf=\xbf'.
$
} 
\begin{proof}[Proof of Claim] Suppose that the injectivity does not hold, i.e. there are $\xbf\neq\xbf'\in X^k$ such that 
\be\label{e:LinearCombination}
\sum_i \alpha_i x_i=\sum_i \alpha_i x_i'.
\ee   
Without loss of generality we can assume that $x_k\neq x_k'$. Thus
\begin{align*}
\f&= \alpha_1 (x_k-x_k')X+\cdots+\alpha_k (x_k-x_k')X\\
\text{(by (\ref{e:LinearCombination}))}\hspace{.5cm}
&\subseteq \alpha_1 (X\cdot X-X\cdot X)+\cdots+\alpha_{k-1} (X\cdot X-X\cdot X)+\left(\sum_{i=1}^{k-1}\alpha_i(x_i-x_i')\right)X\\
&\subseteq \alpha_1 \gen{X}{2}+\cdots+\alpha_{k-1} \gen{X}{2}.
\end{align*}
\end{proof} 

{\bf Claim 2:} {\em Suppose $0,1\in X\subseteq \f$ and $\alpha_i\in \f^{\times}$ such that 
\[
\f=\alpha_1 X+\cdots+\alpha_k X.
\]
Suppose for any $\xbf,\xbf'\in \gen{X}{2}^k$ we have
\[
\sum_i \alpha_i x_i=\sum_i \alpha_i x_i'\Rightarrow \xbf=\xbf'.
\]
Then $X$ is a subfield of $\f$.
}
\begin{proof}[Proof of Claim] It is enough to show $X\cdot X=X$ and $X+X=X$. For any $y,y'\in X$, there is $\xbf\in X^k$ such that 
\[
\alpha_1(y+y')=\sum_i \alpha_i x_i.
\]
Hence $y+y'=x_1\in X$. And so $X$ is closed under addition. Similarly it is closed under multiplication. 
\end{proof}
Now suppose $i_0\le k$ be the largest non-negative integer such that 
\[
\f=\alpha_1'\gen{B}{4^{i_0}}+\cdots+\alpha_{k-i_0}'\gen{B}{4^{i_0}},
\]
for some $\alpha_i'\in \f^{\times}$. If $i_0=k$, we are done. If not, then by Claim 1 for $X=\gen{\gen{B}{4^{i_0}}}{2}$ we have that for any 
$\xbf,\xbf'\in \gen{\gen{B}{4^{i_0}}}{2}^{k-i_0}$ we have
\[
\sum_i \alpha_i' x_i=\sum_i \alpha_i' x_i' \Rightarrow \xbf=\xbf'.
\]
Hence, by Claim 2, $\gen{B}{4^{i_0}}$ is a subfield of $\f$. 
\end{proof}
\begin{lem}\label{l:GradingAreFields}
For any $0<\delta<\vare\ll 1$, $0<\delta'\le \vare^2\delta/4$, $|\f|\gg_{\vare,\delta} 1$, and positive integer $1\ll_{\vare} C$, and any unramified extension $K$ of $\bbq_p$ the following holds:

 Suppose $A\subseteq \pi_{\pfr^N}(\ocal)$ such that 
\begin{enumerate}
\item $\pi_{\pfr}(A)=\f$.
\item $|\pi_{\pfr^i}(A)|\ge |\f|^{i\vare}$ for any $N\delta'\le i\le N$.
\item $0,1\in A$.
\item $|A+A|\le |A||\f|^{N\delta'}$.
\end{enumerate} 
Then $\gr_i(\gen{A}{C})=\f$, for $N\delta \le i\le N$, where 
$\gr_i(X):=\pi_{\pfr}(\{x\in \ocal|\h \pi_{\pfr^N}(\pfr^i x)\in X\})$.  
\end{lem}
\begin{proof}
For any subset $X$ of $\pi_{\pfr^N}(\ocal)$, let 
\[
J(X):=\{k\in \bbz^+|\h \gr_k(X)\neq 0\}. 
\]  
Notice the following observations:
\begin{enumerate}
\item If $j\in J(X)$, then $\gr_j(A X)=\f$. 
\item $J(X_1)+J(X_2)\subseteq J(X_1 X_2)$.
\item $1\in J(A+A-A)$.
\item If $j\in J(X)$, then $j+1\in J((A+A-A)X)$.
\end{enumerate}
The only item that needs a justification is the third one: let $s:\f\rightarrow \pi_{\pfr^2}(A)$ be a section of $\pi_{\pfr}:\pi_{\pfr^2}(A)\rightarrow \f$. Since $K$ is an unramified extension of $\bbq_p$, $\f$ cannot be embedded into $\pi_{\pfr^2}(\ocal)$ as an additive group. Hence there are $x_1,x_2 \in \f$ such that $s(x_1)+s(x_2)-s(x_1+x_2)\neq 0$, which implies that $1\in J(A+A-A)$.
 
By Lemma~\ref{l:RegularSubset}, there is $A'\subseteq A$ such that 
\begin{enumerate}
\item $A'$ is $(m_0,\ldots,m_{N-1})$-regular.
\item $|\pi_{\pfr^i}(A')|\ge |\f|^{i\vare/2}$ for $N(2\delta'/\vare)\le i\le N$.
\end{enumerate}
Since $\gr_0(A)=\f$ and $\gr_1(A+A-A)\neq 0$, as in the proof of Theorem~\ref{t:ScalarSumExpansion} changing $A'$ to a subset of $\sum_6 A-\sum_2 A$ we can assume that $m_0,m_1>1$. 

Let $x_i:=\frac{\log m_i}{\log |\f|}$. Then $0\le x_j\le 1$,
\be\label{e:MoreThanOne}
0,1\in \{i\in [0,N-1]|\h x_i\neq 0\}\subseteq J(A'-A'),
\ee
and 
\be\label{e:Density2}
\sum_{j=0}^i x_j\ge i\vare/2,
\ee
for any $N(2\delta'/\vare) \le i\le N$.

Hence by Lemma~\ref{l:LargeInterval} we have 
\[
[N\delta,N]\cap \bbz\subseteq [N\delta'(4/\vare^2),N] \cap \bbz \subseteq \textstyle \sum_{\lceil 6/\vare\rceil} J(A'-A')\subseteq J(\prod_{\lceil 6/\vare\rceil} (\sum_6 A-\sum_6 A)).
\]

\end{proof}

==> SG_SumProduct_ProofOfBoxDim.tex <==
\subsection{Proof of Theorem~\ref{t:PositiveLowerBoxDimension}.} Let $R$ be the ring generated by $A$. By Lemma ~\ref{lem-bounded-generation-large-mod-all-powers-till-N}, for any positive integers $N\gg_{\vare,d} 1$ and $C\gg_{\vare,d} 1$ there are positive integers $m(N)$ and $n(N)$, $a_N\in \ocal$, and a closed subfield $K_N$ of $K$ with ring of integers $\ocal_N$ such that 
\begin{align}
	n(N) \ll_{\vare,d} N &
	\ll_{\vare,d} n(N)-m(N),
	\\
	\notag
	\pi_{\pfr^{n(N)}}(\ocal_N a_N)&
	\subseteq \pi_{\pfr^{n(N)}}(\gen{A}{C}),
\hspace{1cm} v_{\pfr}(a_N)=m(N),
	\\
	\notag
	|\pi_p(\ocal_N)|&
	\ge |\pi_p(R)|\ge p^{d\vare}.
\end{align}



Since $0,1$ are in $A$, $\{\gen{A}{i}\}_i$ is an increasing sequence of subsets of $R$. 

By assumption for any positive integer $i$ we have $|\pi_{\pfr^i}(A)|\ge |\f|^{i\vare}$. 
